Robust Accelerated Primal-Dual Methods for Computing Saddle Points

We consider strongly-convex-strongly-concave saddle point problems assuming we have access to unbiased stochastic estimates of the gradients. We propose a stochastic accelerated primal-dual (SAPD) algorithm and show that SAPD sequence, generated using constant primal-dual step sizes, linearly converges to a neighborhood of the unique saddle point. Interpreting the size of the neighborhood as a measure of robustness to gradient noise, we obtain explicit characterizations of robustness in terms of SAPD parameters and problem constants. Based on these characterizations, we develop computationally tractable techniques for optimizing the SAPD parameters, i.e., the primal and dual step sizes, and the momentum parameter, to achieve a desired trade-off between the convergence rate and robustness on the Pareto curve. This allows SAPD to enjoy fast convergence properties while being robust to noise as an accelerated method. SAPD admits convergence guarantees for the distance metric with a variance term optimal up to a logarithmic factor -which can be removed by employing a restarting strategy. We also discuss how convergence and robustness results extend to the convex-concave setting. Finally, we illustrate our framework on distributionally robust logistic regression problem.

==> defs.tex <==
% MATH SUMBOLS AND RELATED MACROS
\def\grad{\nabla}
\def\noi{\noindent}
\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bd{\mathbf{d}}
\def\be{\mathbf{e}}
\def\bff{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
\def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}  %{\mbox{\boldmath $\lambda$}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bU{\mathbf{U}}
\def\bT{\mathbf{T}}
\def\bY{\mathbf{Y}}
\def\bX{\mathbf{X}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bZ{\mathbf{Z}}
\def\bo{\mathbf{0}}

\def\e{{\boldsymbol{\epsilon}}}
\def\l{{\boldsymbol{\lambda}}}
\def\g{{\boldsymbol{\gamma}}}
\def\G{{\boldsymbol{\Gamma}}}
\def\L{{\boldsymbol{\Lambda}}}
\def\D{{\boldsymbol{\Delta}}}
\def\a{{\boldsymbol{\alpha}}}
\def\m{{\boldsymbol{\mu}}}
\def\n{{\boldsymbol{\nu}}}
%\def\S{{\boldsymbol{\Sigma}}}
\def\p{{\boldsymbol{\pi}}}
\def\th{{\boldsymbol{\theta}}}
\def\Th{{\boldsymbol{\Theta}}}
\def\x{{\boldsymbol{\xi}}}
\def\b{{\boldsymbol{\beta}}}
\def\r{{\boldsymbol{\rho}}}
\def\z{{\boldsymbol{\zeta}}}
\def\ph{{\boldsymbol{\phi}}}
\def\ps{{\boldsymbol{\psi}}}
\def\pis{\pi^{\star}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}



\def\mA{\mathbb{A}}
\def\mB{\mathbb{B}}
\def\mC{\mathbb{C}}
\def\mD{\mathbb{D}}
\def\mE{\mathbb{E}}
\def\mF{\mathbb{F}}
\def\mG{\mathbb{G}}
\def\mH{\mathbb{H}}
\def\mI{\mathbb{I}}
\def\mJ{\mathbb{J}}
\def\mK{\mathbb{K}}
\def\mL{\mathbb{L}}
\def\mM{\mathbb{M}}
\def\mN{\mathbb{N}}
\def\mO{\mathbb{O}}
\def\mP{\mathbb{P}}
\def\mQ{\mathbb{Q}}
\def\mR{\mathbb{R}}
\def\mS{\mathbb{S}}
\def\mT{\mathbb{T}}
\def\mU{\mathbb{U}}
\def\mV{\mathbb{V}}
\def\mW{\mathbb{W}}
\def\mX{\mathbb{X}}
\def\mY{\mathbb{Y}}
\def\mZ{\mathbb{Z}}

\def\eq{\[}
\def\en{\]}

\def\smskip{\smallskip}
\def\sep#1{ \hskip -5pt & #1 & \hskip -5 pt}
\def\texitem#1{\par\smskip\noindent\hangindent 25pt
               \hbox to 25pt {\hss #1 ~}\ignorespaces}

% mathematical constructs
\def\abs#1{\left|#1\right|}
\def\norm#1{\|#1\|}
\def\vec#1{\left(\!\begin{array}{c}#1\end{array}\!\right)}
\def\bmat#1{\left[\begin{array}{cc}#1\end{array}\right]}

% some traditional definitions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{eqnarray}}
\newcommand{\EEQ}{\end{eqnarray}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

% arash added these two
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}

\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{\mathbb{C}}

% Re & Im
%\renewcommand{\Re}{\mathop{\bf Re}}
%\renewcommand{\Im}{\mathop{\bf Im}}

% lin alg stuff
\newcommand{\Span}{\mbox{\textrm{span}}}
%\newcommand{\Range}{\mbox{\textrm{range}}}
\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Nullspace}{\mbox{\textrm{nullspace}}}
\newcommand{\Rank}{\mathop{\bf rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\detr}{\mathop{\bf det}}
%\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}

% probability stuff
\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\erf}{\mathop{\bf erf}}
\def\Pr{\mathbb{P}}

% convexity & optimization stuff
\def\co{{\mathop {\bf cone}}}
\def\conv{\mathop {\bf conv}}
%\def\var#1{\mathop{\bf Var}\big[#1\big]}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}

%\newcommand{\QED}{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
%\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\epi}{\mathop{\bf epi}}
\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\ri}{\mathop{\bf ri}}
\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\Vol}{\mathop{\bf vol}}

\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bdry}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}

%the following ones seem way too specialized to be here...
\newcommand{\xopt}{x^{\rm opt}}
\newcommand{\Xb}{{\mbox{\bf X}}}
\newcommand{\xst}{x^\star}
\newcommand{\varphist}{\varphi^\star}
\newcommand{\lambdast}{\lambda^\star}
\newcommand{\Zst}{Z^\star}
\newcommand{\fstar}{f^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\xc}{x^\star}
\newcommand{\lambdac}{\lambda^\star}
\newcommand{\lambdaopt}{\lambda^{\rm opt}}

%generalized inequalities for cvx book
\newcommand{\geqK}{\mathrel{\succeq_K}}
%\newcommand{\geqq}{\mathrel{\succeq_{\cQ}}}
\newcommand{\gK}{\mathrel{\succ_K}}
\newcommand{\leqK}{\mathrel{\preceq_K}}
\newcommand{\lK}{\mathrel{\prec_K}}
\newcommand{\geqKst}{\mathrel{\succeq_{K^*}}}
\newcommand{\gKst}{\mathrel{\succ_{K^*}}}
\newcommand{\leqKst}{\mathrel{\preceq_{K^*}}}
\newcommand{\lKst}{\mathrel{\prec_{K^*}}}
\newcommand{\geqL}{\mathrel{\succeq_L}}
\newcommand{\gL}{\mathrel{\succ_L}}
\newcommand{\leqL}{\mathrel{\preceq_L}}
\newcommand{\lL}{\mathrel{\prec_L}}
\newcommand{\geqLst}{\mathrel{\succeq_{L^*}}}
\newcommand{\gLst}{\mathrel{\succ_{L^*}}}
\newcommand{\leqLst}{\mathrel{\preceq_{L^*}}}
\newcommand{\lLst}{\mathrel{\prec_{L^*}}}
\def\join{\vee}
\def\meet{\wedge}

% colored text
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\tri#1{\textcolor{#1}{$\blacktriangleright$}}

%% macros

\newif\ifpagenumbering
\pagenumberingtrue
\newcommand{\firstpagenumber}{1}
\pagenumberingfalse

%
%  Conditionals for generating different versions
%
% \newif\ifabstract
% \newif\ifjournal
% \newcommand{\mnote}[1]{{\tiny\marginpar[#1]{#1}}}
\newsavebox{\theorembox}
\newsavebox{\lemmabox}
% \newsavebox{\claimbox}
% \newsavebox{\factbox}
\newsavebox{\defnbox}
% \newsavebox{\corollarybox}
% \newsavebox{\propositionbox}
% \newsavebox{\examplebox}
% \newsavebox{\exercisebox}
% \newsavebox{\problembox}
% \newsavebox{\conjecturebox}
% \newsavebox{\oqbox}
%\newsavebox{\remarkbox}
\newsavebox{\assbox}
\savebox{\theorembox}{\noindent\bf Theorem}
\savebox{\lemmabox}{\noindent\bf Lemma}
% \savebox{\claimbox}{\noindent\bf Claim}
% \savebox{\factbox}{\noindent\bf Fact}
\savebox{\defnbox}{\noindent Definition}
% \savebox{\corollarybox}{\noindent\bf Corollary}
% \savebox{\propositionbox}{\noindent\bf Proposition}
% \savebox{\examplebox}{\noindent\bf Example}
% \savebox{\exercisebox}{\noindent\bf Exercise}
% \savebox{\problembox}{\noindent\bf Problem}
% \savebox{\conjecturebox}{\noindent\bf Conjecture}
%\savebox{\remarkbox}{\noindent\bf Remark}
% \savebox{\oqbox}{\noindent\bf Open Question}
%\savebox{\assbox}{\noindent\bf Assumption}
%\newtheorem{assumption}{\usebox{\assbox}}
%\newtheorem{theorem}{\usebox{\theorembox}}
%\newtheorem{lemma}{\usebox{\lemmabox}}
% \newtheorem{claim}{\usebox{\claimbox}}
% \newtheorem{fact}{\usebox{\factbox}}
%\newtheorem{remark}{\usebox{\remarkbox}}[section]
% \newtheorem{corollary}{\usebox{\corollarybox}}
% \newtheorem{proposition}[theorem]{\usebox{\propositionbox}}
% \newtheorem{exercise}{\usebox{\exercisebox}}
% \newtheorem{example}{\usebox{\examplebox}}
% \newtheorem{problem}{\usebox{\problembox}}
% \newtheorem{conjecture}{\usebox{\conjecturebox}}
% \newtheorem{oq}{\usebox{\oqbox}}
\newtheorem{defn}{\usebox{\defnbox}}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt depth 1.5pt
\hskip 1pt}}
%\newtheorem{exprime}{Example}%[section]
%\newenvironment{example}{\noindent\exprime\em {\vspace{-0.05 in}}}{
%\hfill $\blackslug$ \par \addvspace{\bigskipamount}{\vspace{0in}}}
%% \newenvironment{example}{\noindent\exprime\em {\vspace{-0.05 in}}}{
%% \hfill $\blackslug$ \par \addvspace{\bigskipamount}{\vspace{0in}}}

%Miscellaneous commands for proofs
%\newcommand{\qed}{\mbox{}\hspace*{\fill}\nolinebreak\mbox{$\rule{0.7em}{0.7em}$}}
\newcommand{\proc}[1]{\textnormal{\scshape#1}}
\usepackage{soul}
%\newenvironment{proof}{\par{\noi \bf Proof: }}{\(\qed\) \par}
% \newenvironment{proofsketch}{\par{\noi \bf Proof Sketch:}}{\(\qed\) \par}
% \newenvironment{solutionsketch}{\par{\bf Solution Sketch:}}{\(\qed\) \par}
% \newenvironment{deffproof}[1]{\par{\bf Proof #1:}}{\(\qed\) \par}
% \newcommand{\case}[1]{{\small \sc Case #1:}}
% \newcommand{\subcase}[1]{{\em Case #1:}\/}

% \renewcommand{\hat}[1]{\widehat{#1}}
% \newcommand{\opt}{\mbox{\footnotesize\sc opt}}
% \newcommand{\parent}{\mbox{\sc parent}}
% \newcommand{\precstar}{\stackrel{\mbox{\raisebox{-0.5ex}[0pt][0pt]{\tiny$\star$}}}{\prec}}

\usepackage[normalem]{ulem}
\DeclareUnicodeCharacter{2212}{~}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage[utf8]{inputenc}
\usepackage{url}
\usepackage{amssymb}
\usepackage{hyperref}
\usepackage{verbatim}
\usepackage{amsmath}
\usepackage{indentfirst}
\usepackage{float}%use [h] to fix postion of a figure
\usepackage{xcolor}
\usepackage{comment}
\usepackage{graphicx}
\usepackage{subfigure}
% \usepackage{subcaption}
% \captionsetup{compatibility=false}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added by NSA on 06/25/2020 to make \todo work better
\usepackage{breqn}
\usepackage{todonotes}
\setlength\marginparwidth{1in}
\usepackage{etoolbox}
\makeatletter
\patchcmd{\@addmarginpar}{\ifodd\c@page}{\ifodd\c@page\@tempcnta\m@ne}{}{}
\makeatother
\reversemarginpar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added by NSA on 08/06/2020 to use \MoveEqLeft[4] (moves 4em to the left) and \MoveEqLeft for long equations in align
\usepackage{mathtools}
\allowdisplaybreaks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added by NSA on 10/27/2021 to use \mathbbm{1} for indicator functions
\usepackage{bbm}
\usepackage{bbding}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Added by Xuan on 06/21/2021 to use \barbelow
\usepackage{stackengine}
\newcommand\barbelow[1]{\stackunder[1.2pt]{$#1$}{\rule{.8ex}{.075ex}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi
\DeclareMathOperator*{\argmax}{\textbf{argmax}}
\DeclareMathOperator*{\argmin}{\textbf{argmin}}
\def\sa#1{\textcolor{red}{#1}}
\def\saa#1{\textcolor{red}{#1}}
\def\fprod#1{\left\langle#1\right\rangle}
\def\prox#1{\mathbf{prox}_{#1}}
\def\mg#1{\textcolor{blue}{#1}}
\def\xzh#1{\textcolor{orange}{#1}}
\def\nsa#1{\todo[size=footnotesize]{NSA:~#1}}
\def\xuan#1{\todo[size=footnotesize]{XUan:~#1}}
\newcommand{\mtodo}[1]{\todo[size=footnotesize,color=purple!20]{{\bf M:} #1}}
\newcommand{\xtodo}[1]{\todo[size=footnotesize,color=blue!20]{{\bf X:} #1}}
\def\dd#1{\textcolor{purple}{#1}}
\def\xuan#1{\textcolor{black}{#1}}
\def\newcomment#1{\textcolor{brown}{#1}}
\input{defs.tex}
\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}


% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\crefname{assumption}{Assumption}{Assumption}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{ROBUST PRIMAL-DUAL METHODS FOR COMPUTING SADDLE POINT}{X.Zhang, N.S.Aybat and M.Gürbüzbalaban}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Robust \mg{Accelerated} Primal-Dual Methods\\ for Computing Saddle Points
%\thanks{This work was funded by ONR Grants N00014-21-1-2271 and N00014-21-1-2244.}
%\funding{This work was funded by }
}

% Authors: full names plus addresses.
\author{
XUAN ZHANG\thanks{Department of Industrial and Manufacturing Engineering, Pennsylvania State University, University Park, PA,USA. (\email{xxz358@psu.edu}, \email{nsa10@psu.edu}).}
\and
Necdet Serhat Aybat\footnotemark[1]
\and
Mert Gürbüzbalaban
\thanks{Department of Management Science and Information Systems, Rutgers University, Piscataway, NJ, USA.\email{mg1366@rutgers.edu}}
}

\usepackage{amsopn}

\DeclareMathOperator{\diag}{diag}

\newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}}
%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
